Real-Time Neural Hair G-Buffer Anti-Aliasing

We propose a lightweight real-time method for reconstructing strand-based hair G-Buffers from severely undersampled rasterized inputs. Our pipeline first applies neural spatial reconstruction and temporal accumulation to recover hair coverage, i.e., fractional hair visibility within a pixel, and tangent. It then uses a tangent-guided reconstruction step to complete the position, which is subsequently used for physically based deferred hair shading. We evaluate our method across a diverse set of hairstyles, including straight, wavy, afro, and ponytail styles, under both static and dynamic scenarios. Our method achieves higher hair reconstruction quality than general industrial neural reconstruction solutions such as DLSS and FSR.

==> Alg_curvature_center.tex <==
% \RestyleAlgo{ruled}
% \begin{algorithm}[ht!]
% \caption{Curvature Estimation}
% \DontPrintSemicolon
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor[RGB]{0 128 64}{#1}}
% \SetCommentSty{mycommfont} 
% \label{alg:robust_curvature}
% %\Require Position map $\mathbf{P}\in\mathbb{R}^{H\times W\times 2}$, validity map $\mathbf{D}$, \kui{validity map?} radius $r$, minimum curvature $\kappa_{\min}$, area threshold $\epsilon_A$
% %\Ensure Curvature map $\boldsymbol{\kappa}$, center map $\mathbf{C}$

% \todo{update}

% \tcp{Initialization}
% $\kappa_{ij}\gets \kappa_{\min}$\\
% $\mathbf{C}_{ij}\gets \mathbf{0}$

% \For{$\pp \in \DD(\pp)>0$}{
%     $\mathbf{p}_0 \gets \PP(\pp)$\\
%     $\mathcal{N}_{ij}\gets \{\mathbf{P}_{uv}: |u-i|\le r,\ |v-j|\le r,\ (u,v)\neq(i,j),\ \mathbf{D}_{uv}>0\}$

%     \If{$|\mathcal{N}_{\pp}|<2$}{
%         \textbf{continue}
%     }

%     Sort $\mathcal{N}_{ij}$ by distance to $\mathbf{p}_0$

%     Select the first pair $(\mathbf{p}_a,\mathbf{p}_b)$ such that the triangle $(\mathbf{p}_0,\mathbf{p}_a,\mathbf{p}_b)$ has area $A>\epsilon_A$

%     \If{no such pair exists}{
%         \textbf{continue}
%     }

%     \tcp{compute side lengths}
%     $a=\|\mathbf{p}_a-\mathbf{p}_b\|$\\
%     $b=\|\mathbf{p}_0-\mathbf{p}_b\|$\\
%     $c=\|\mathbf{p}_0-\mathbf{p}_a\|$

%     \tcp{Compute triangle area}
%     $A=\sqrt{s(s-a)(s-b)(s-c)}$\\
%     $s=\frac{a+b+c}{2}$

%     \tcp{Estimate curvature by the circumcircle}
%     $\kappa_{ij} = \frac{1}{R} =\frac{4A}{abc}$

%     Compute circumcenter $\mathbf{C}_{ij}$ of $(\mathbf{p}_0,\mathbf{p}_a,\mathbf{p}_b)$
% }

% %\Return $\boldsymbol{\kappa}, \mathbf{C}$
% \end{algorithm}

\RestyleAlgo{ruled}
\begin{algorithm}[ht!]
\caption{Curvature Estimation}
\DontPrintSemicolon
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor[RGB]{0 128 64}{#1}}
\SetCommentSty{mycommfont} 
\label{alg:robust_curvature}

\KwIn{Pixel cordinates map $\PP\in\mathbb{R}^{H\times W\times 2}$, validity map $\DD$, search radius $r$, minimum curvature $\kappa_{\min}$, area threshold $\epsilon_A$, far-center distance $C_{\mathrm{far}}$}
\KwOut{Curvature map $\boldsymbol{\kappa}$, curvature center map $\CC$}

\tcp{Initialization}
Initialize $\kappa_{\pp}\gets \kappa_{\min}$ and $\CC_{\pp}\gets \mathbf{0}$ for all pixels $\pp$\;

\For{each pixel $\pp=(i,j)$ such that $\DD_{\pp}>0$}{
    $\mathbf{p}_0 \gets \PP_{\pp}$\;

    $\mathcal{N}_{\pp}\gets
    \{\PP_{uv}: |u-i|\le r,\ |v-j|\le r,\ (u,v)\neq(i,j),\ \DD_{uv}>0\}$\;

    \If{$|\mathcal{N}_{\pp}|<2$}{
        $\CC_{\pp}\gets \mathbf{p}_0 + C_{\mathrm{far}}[1,0]^T$\;
        \textbf{continue}\;
    }

    Sort $\mathcal{N}_{\pp}$ by Euclidean distance to $\mathbf{p}_0$\;

    $\mathrm{found}\gets \mathrm{false}$\;

    \For{each ordered pair $(\mathbf{p}_a,\mathbf{p}_b)$ from $\mathcal{N}_{\pp}$}{
        \tcp{Compute side lengths}
        $a=\|\mathbf{p}_a-\mathbf{p}_b\|$\;
        $b=\|\mathbf{p}_0-\mathbf{p}_b\|$\;
        $c=\|\mathbf{p}_0-\mathbf{p}_a\|$\;

        \tcp{Compute triangle area}
        $s=\frac{a+b+c}{2}$\;
        $A=\sqrt{\max(s(s-a)(s-b)(s-c),0)}$\;

        \If{$A>\epsilon_A$}{
            $\mathrm{found}\gets \mathrm{true}$\;
            \textbf{break}\;
        }
    }

    \If{$\mathrm{found}=\mathrm{false}$}{
        $\mathbf{p}_1\gets$ the nearest point in $\mathcal{N}_{\pp}$\;
        $\mathbf{v}\gets \mathbf{p}_1-\mathbf{p}_0$\;
        $\mathbf{n}\gets [-v_y,v_x]^T / \|\mathbf{v}\|$\;
        $\kappa_{\pp}\gets \kappa_{\min}$\;
        $\CC_{\pp}\gets \mathbf{p}_0 + C_{\mathrm{far}}\mathbf{n}$\;
        \textbf{continue}\;
    }

    \tcp{Estimate curvature by the circumcircle}
    $\kappa_{\pp} \gets \frac{1}{R} = \frac{4A}{abc}$\;

    Compute circumcenter $\CC_{\pp}$ of $(\mathbf{p}_0,\mathbf{p}_a,\mathbf{p}_b)$\;
}

\Return{$\boldsymbol{\kappa}, \CC$}
\end{algorithm}

==> Alg_tangent_guided_recosntruction.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[ht!]
\caption{Bidirectional Position Reconstruction}
\DontPrintSemicolon
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor[RGB]{0 128 64}{#1}}
\SetCommentSty{mycommfont} 
\label{alg:tangent-guided-reconstuction}
\tcp{Pixel Classification}
$\mathbf{M}_\text{invalid} \leftarrow \{\pp : \CC(\pp)>0 \;\wedge\; \TT(\pp)>0 \;\wedge\; \PP(\pp)=\mathbf{0}\}$\\
$\mathbf{M}_\text{valid}   \leftarrow \{\pp : \CC(\pp)>0 \;\wedge\; \PP(\pp)\neq\mathbf{0}\}$\\
$\mathbf{M}_\text{hair}    \leftarrow \mathbf{M}_\text{valid} \cup \mathbf{M}_\text{invalid}$

\tcp{Depth Impainting}
$\mathbf{M}_\text{Impaint} \leftarrow \{\pp : \CC(\pp)>0 \;\wedge\; \mathbf{D}(\pp))>0\}$\\
\For{each $\pp \notin \mathbf{M}_\mathrm{Impaint}$}{
    $\pp^* \leftarrow \arg\min_{\qq\in\mathbf{M}_\text{Impaint}} \|\pp-\qq\|_2$\\
    $\DD(\pp) \leftarrow \DD(\pp^*)$
}
\tcp{Bidirectional Position Reconstruction}
\tcp{Stage I: Per-pixel step size computation}
$l_{\pp} = \sqrt{\left({\DD(\pp)}/{f_x}\right)^2 + \left({\DD(\pp)}/{f_y}\right)^2}$ \tcp{camera intrinsics $(f_x, f_y)$}

\tcp{Stage II: Screen-space curvature center estimation}
$\xx_\text{screen} \leftarrow \text{\fontfamily{lmss}\selectfont ScreenPos}(H, W)$\\
$\mathbf{c} \leftarrow \text{\fontfamily{lmss}\selectfont CurvatureCenter}(\xx_\text{screen},\ \mathbf{C},\ r{=}3)$

\tcp{Stage III: Screen space Tangent Projection}
$\tt_\text{screen} \leftarrow \text{Project}(\TT(\pp),\ \mathbf{V})$ \tcp{view-projection matrix $\VV$}
$\tt_\text{screen} \leftarrow \tt_\text{screen} / \|\tt_\text{screen}\|$\\
$\hat{\mathbf{P}} \leftarrow \mathbf{P}$

\tcp{Stage IV: Backward repair for missing pixels}
\For{each $\pp \in \mathbf{M}_\mathrm{invalid}$}{
    % $\ss^\star \leftarrow \arg\min_{s \in\mathcal{N}_{\pp}\cap\mathbf{M}_\text{valid}} \|\xx_\text{screen}(\ss) - \cc_{\pp}\|_2 $\\
    $\ss^\star \leftarrow \arg\min_{\ss \in \mathcal{N}_{\pp}\cap\mathbf{M}_\text{valid}} \left\|\xx_\text{screen}(\ss)-\cc_{\pp}\right\|_2$\\
    % $\PP^{\star}(\pp) = \PP(\ss^\star) + l_{\pp}\,\TT^\star(\pp)$
    $\PP^{\star}(\pp) \leftarrow \PP(\ss^\star) + l_{\pp}\,\TT(\pp)$
}

\tcp{Stage V: Forward voting from valid pixels}
\For{each target pixel $\pp \in \mathbf{M}_\mathrm{hair}$}{
    \For{each source pixel $\ss \in \mathcal{N}_\pp\cap\mathbf{M}_\mathrm{valid}$}{
        \If{$\left|
\TT_{\mathrm{screen}}(\ss)\cdot
\frac{\pp-\ss}{\|\pp-\ss\|_2}
\right|
\geq
\cos\theta_{\max}$}{
            add $\PP(\ss) + l_{\ss}\,\TT(\ss)$ to a stack $\mathcal{S}$\\
            keep top-$K$ by depth
        }
    }
}
\For{each $\pp \in \mathcal{S}$}{
    $\PP^{\star}(\pp)
=
\arg\min_{\qq \in \mathcal{C}_{\pp}}\text{\fontfamily{lmss}\selectfont depth}(\qq)$
}
% \todo{update the following two lines}

% $\mathbf{M}_\text{valid} \leftarrow \mathbf{M}_\text{valid} \cup \{t\in\mathbf{M}_\text{invalid}: \hat{\mathbf{P}}_\text{new}[t]\neq\hat{\mathbf{P}}[t]\}$\\
% $\hat{\mathbf{P}} \leftarrow \hat{\mathbf{P}}_\text{new}$

$\mathbf{M}_\mathrm{changed}
\leftarrow
\{\pp\in\mathbf{M}_\mathrm{hair}:
\|\hat{\PP}_\mathrm{new}(\pp)-\hat{\PP}(\pp)\|_2>\epsilon\}$\\

\If{$\mathbf{M}_\mathrm{changed}=\emptyset$}{
    \textbf{break}
}

$\hat{\PP}\leftarrow\hat{\PP}_\mathrm{new}$\\

$\mathbf{M}_\mathrm{filled}
\leftarrow
\mathbf{M}_\mathrm{invalid}\cap\mathbf{M}_\mathrm{changed}$\\

$\mathbf{M}_\mathrm{valid}
\leftarrow
\mathbf{M}_\mathrm{valid}\cup\mathbf{M}_\mathrm{filled}$\\

$\mathbf{M}_\mathrm{invalid}
\leftarrow
\mathbf{M}_\mathrm{invalid}\setminus\mathbf{M}_\mathrm{filled}$

%\Return $\hat{\mathbf{P}}$
\end{algorithm}


==> Fig_network_architecture.tex <==
\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.45\textwidth]{network_architecture_draft.png}
    \caption{Overview of our neural network. \todo{update}}
    \Description{}
    % \vspace{-15pt}
    \label{fig:network_architecture}
\end{figure}

==> Table_ablation.tex <==
\begin{table}[hbt]
\centering
\small
\caption{Ablation of our pipeline.} 
\label{tab:ablation}
\renewcommand{\tabcolsep}{0.05cm}
\begin{tabular}{lccccccc}
\toprule
Method 
& MSE$\downarrow$ 
& PSNR$\uparrow$ 
& SSIM$\uparrow$ 
& LPIPS$\downarrow$
& FLIP$\downarrow$
& FVVDP$\uparrow$
& Time$\downarrow$ (ms)\\
\midrule
Input & 0.0111 & 19.72 & 0.9433 & 0.0513 & 0.0192 & 8.40 & -- \\
w/o Spatial & 0.0077 & 21.25 & 0.9531 & 0.0385 & 0.0174 & 8.37 & 0.4\\
w/o Temporal & 0.0021 & 27.07 & 0.9706 & 0.0214 & 0.0084 & 9.16 & 0.7\\
w/o Analytic & 0.0139 & 18.65 & 0.9387 & 0.0370 & 0.0185 & 8.22 & 0.9\\
Ours  & \textbf{0.0014} & \textbf{28.57} & \textbf{0.9756} & \textbf{0.0155} & \textbf{0.0075} & \textbf{9.27} & 1.0\\
\bottomrule
\end{tabular}
\end{table}

==> Table_ablation_analytic.tex <==
\begin{table}[hbt]
\centering
\small
\caption{Ablation of analytic filtering, note that the metrics are for the position map instead of the deferred shading result.} 
\label{tab:ablation_analytic}
\renewcommand{\tabcolsep}{0.05cm}
\begin{tabular}{lcccccc}
\toprule
Method 
& MSE$\downarrow$ 
& PSNR$\uparrow$ 
& SSIM$\uparrow$ 
& LPIPS$\downarrow$
& FLIP$\downarrow$
& Time$\downarrow$\\
\midrule
Input & 0.0136 & 18.67 & 0.8735 & 0.1498 & 0.1102 & -- \\
Backward & 0.0014 & 28.66 & 0.9508 & 0.0449 & 0.0627 & 0.04\\
Forward & 0.0044 & 23.54 & 0.9460 & 0.0456 & 0.0481 & 0.06\\
Both  & \textbf{0.0011} & \textbf{29.40} & \textbf{0.9728} & \textbf{0.0177} & \textbf{0.0315} & 0.10\\
\bottomrule
\end{tabular}
\end{table}

==> Table_color_light.tex <==
\begin{table}[hbt]
\centering
\small
\caption{Masked-hair metrics of difference color and light of Fig. 7 in the main paper.} 
\label{tab:appearance}
\renewcommand{\tabcolsep}{0.1cm}
\begin{tabular}{lcccccc}
\toprule
Method 
& MSE$\downarrow$ 
& PSNR$\uparrow$ 
& SSIM$\uparrow$ 
& LPIPS$\downarrow$
& FLIP$\downarrow$
& Time$\downarrow$\\
\midrule

Input & 0.0524 & 12.80 & 0.8810 & 0.1186 & 0.0889 & -- \\
TAA   & 0.0232 & 16.35 & 0.9157 & 0.0762 & 0.0680 & 0.1\\
FSR   & 0.0243 & 16.15 & 0.9088 & 0.0790 & 0.0658 & 0.5\\
DLSS  & 0.0200 & 17.00 & 0.9154 & 0.0676 & 0.0569  & 0.5\\
Ours  & \textbf{0.0027} & \textbf{25.72} & \textbf{0.9644} & \textbf{0.0198} & \textbf{0.0227} & 0.8\\

\midrule

Input & 0.0405 & 13.93 & 0.8823 & 0.1182 & 0.0595 & -- \\
TAA   & 0.0151 & 18.21 & 0.9284 & 0.0533 & 0.0456 & 0.1\\
FSR   & 0.0176 & 17.55 & 0.9155 & 0.0688 & 0.0454 & 0.5\\
DLSS  & 0.0144 & 18.43 & 0.9235 & 0.0585 & 0.0455  & 0.5\\
Ours  & \textbf{0.0021} & \textbf{26.74} & \textbf{0.9653} & \textbf{0.0180} & \textbf{0.0138} & 0.8\\

\midrule

Input & 0.0318 & 14.97 & 0.8845 & 0.1200 & 0.0338 & -- \\
TAA   & 0.0102 & 19.92 & 0.9347 & 0.0591 & 0.0283 & 0.1\\
FSR   & 0.0124 & 19.07 & 0.9218 & 0.0772 & 0.0289 & 0.5\\
DLSS  & 0.0098 & 20.08 & 0.9338 & 0.0583 & 0.0289  & 0.5\\
Ours  & \textbf{0.0018} & \textbf{27.43} & \textbf{0.9659} & \textbf{0.0206} & \textbf{0.0073} & 0.8\\

\midrule

Input & 0.0381 & 14.19 & 0.8866 & 0.1115 & 0.0565 & -- \\
TAA   & 0.0165 & 17.81 & 0.9288 & 0.0620 & 0.0468 & 0.1\\
FSR   & 0.0172 & 17.65 & 0.9201 & 0.0697 & 0.0467 & 0.5\\
DLSS  & 0.0142 & 18.47 & 0.9292 & 0.0582 & 0.0465  & 0.5\\
Ours  & \textbf{0.0024} & \textbf{26.18} & \textbf{0.9644} & \textbf{0.0201} & \textbf{0.0149} & 0.8\\

\midrule

Input & 0.017639 & 17.54 & 0.9475 & 0.0565 & 0.0855 & -- \\
TAA   & 0.009549 & 20.20 & 0.9594 & 0.0361 & 0.0809 & 0.1\\
FSR   & 0.010558 & 19.76 & 0.9570 & 0.0383 & 0.0806 & 0.5\\
DLSS  & 0.009678 & 20.14 & 0.9599 & 0.0329 & 0.0791  & 0.5\\
Ours  & \textbf{0.001877} & \textbf{27.27} & \textbf{0.9786} & \textbf{0.0098} & \textbf{0.0299} & 0.8\\

\bottomrule
\end{tabular}
\end{table}

==> Table_compare.tex <==
\begin{table}[hbt]
\centering
\small
\caption{Quantitative comparison with \cite{Currius2022}. Note that the results of \citet{Currius2022} with their best model and ours for timing on the table were obtained on an Nvidia RTX 2060.
%; for fairness, we report our time cost on the same device. 
} 
\label{tab:comparison_i3d}
\renewcommand{\tabcolsep}{0.05cm}
\begin{tabular}{lcccccc}
\toprule
Method 
& MSE$\downarrow$ 
& PSNR$\uparrow$ 
& SSIM$\uparrow$ 
& LPIPS$\downarrow$
& FLIP$\downarrow$
& Time$\downarrow$ (ms)\\
\midrule
\citet{Currius2022} & 0.0033 & 24.78 & 0.9251 & 0.0622 & 0.0247 & 20.3 \\
Ours  & \textbf{0.0010} & \textbf{30.06} & \textbf{0.9832} & \textbf{0.0094} & \textbf{0.0105} & 3.6\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> Table_performance.tex <==
\begin{table}[hbt]
\centering
\small
\caption{Performance of our method.} 
\label{tab:performance}
\renewcommand{\tabcolsep}{0.15cm}
\begin{tabular}{lc}
\toprule
 
& Time \\
\midrule
Spatial Module & 0.6 \\
Temporal Accumulation  & 0.3 \\
Analytic Filtering  & 0.1 \\
\bottomrule
Total  & 1.0
\end{tabular}
\end{table}

==> bkgd_anony.tex <==


\section{Related work}

%This section briefly reviews prior works on hair rendering and denoising.

\paragraph{Hair Rendering}

\citet{KajiyaK89} introduced the first physically based analytic hair shading model. This was later extended by \citet{MarschnerJCWH03} into the widely used hair BCSDF model, which decomposes scattering inside dielectric fibers into the $R$, $TT$, and $TRT$ modes. Since then, many works have extended this model, including the addition of a diffuse term for improved data fitting~\cite{ZinkeRLWAK09}, artist-friendly lobe decompositions~\cite{Sadeghi2010}, additional lobes for improved energy conservation and high-order scattering~\cite{dEonFHLA11, ChiangBTB16}, and extensions to elliptical hairs, animal fur, and microfacet-based scattering~\cite{Yan2015, Khungurn2017, Huang2022hair}. More recently, wave-optics models have been proposed to capture the colorful glints of hair and fur~\cite{Xia2020, Xia2023}.

Efficient approximation of multiple scattering is critical for realistic strand-based rendering. Prior work has explored photon mapping with volumetric radiance storage~\cite{MoonM06, moon08}, neural prediction of high-order scattering~\cite{kt2023}, and dual scattering for real-time rendering~\cite{ZinkeYWK08, Yuksel2008}. \citet{Huang2025Knit} further enable efficient multiple-scattering approximation with textured strand details via precomputed dual-scattering corrections.
%for yarn with fiber-level detail via precomputed dual-scattering corrections. \zahra{we don't have the definition of yarn and fiber for "hair", how about just say: "multiple-scattering approximation with textured details"?}

To further accelerate rendering, aggregation models have been developed to represent clusters of fibers or hairs using coarser primitives. \citet{Koh2001} pioneered the use of polygon strips with alpha maps to represent clusters of hair strands for real-time applications; this approach remains widely used in the game industry~\cite{YIbing2016}. To better approximate the aggregated scattering behavior within fiber bundles, \citet{MontazeriGZJ20, Montazeri2021} modeled woven and knitted structures using normal mapping and a specialized BSDF with separate surface and body components. \citet{ZhuZWXY22, ZhuZJYA23} later introduced neural and analytical aggregated BCSDF models for fiber bundles and yarns, respectively. \citet{Bhokare2024} generated hair strand geometry on-the-fly based on \emph{hair mesh}~\cite{Yuksel2009, wu2016}, greatly reducing storage and memory bandwidth requirements for real-time hair rendering. More recently, \citet{Huang2025HairLoD} presented a real-time strand-based rendering framework with seamless level-of-detail transitions, using an aggregated BCSDF to preserve both single- and multiple-scattering effects within hair clusters. 

While many approaches have been proposed to improve the performance of strand-based rendering, including hair level-of-detail (LoD), aggregated models, and dual scattering, the intrinsic geometric nature of hair remains challenging: its width is often smaller than a screen pixel, which requires a large number of samples per pixel to achieve denoised results.


\paragraph{Hair Denoising}
Anti-aliasing and reconstruction are fundamental problems in real-time rendering. Supersample anti-aliasing (SSAA) mitigates aliasing by full-image supersampling at high cost, whereas multisample anti-aliasing (MSAA) improves geometric edge quality while reducing shading noise. Post-process filters, such as fast approximate anti-aliasing (FXAA)~\cite{Lottes2009FXAA}, provide efficient edge smoothing but may blur fine details. Temporal methods such as temporal anti-aliasing (TAA)~\cite{Yang2020taa} improve both anti-aliasing and denoising through cross-frame accumulation, but can introduce ghosting under motion or disocclusion. More recently, neural reconstruction methods such as deep learning super sampling (DLSS) 4~\cite{nvidia2025dlss4} and AMD FidelityFX Super Resolution (FSR)~\cite{amd_fsr} have combined temporal information with learned super-resolution to improve image quality. However, while these techniques work well for general geometry, they are less effective for high-frequency structures such as hair, where aliasing artifacts can persist even after edge detection and filtering.

In strand-based hair rendering, simply enabling MSAA is insufficient to eliminate aliasing and also increases rendering cost due to severe overdraw. To address this, the industrial solution~\cite{tafuri2019strand} adopts a pipeline in which all hair strands are first rasterized in a lightweight MSAA pass into the visibility buffer and then processed by a sample deduplication, so that only distinct samples within each pixel are shaded to produce the anti-aliased result. This pipeline has been widely adopted in modern game engines~\cite{unrealengine, Kulikov2025strand}. \citet{fu2023} proposed an elliptical kernel designed to suppress noise while preserving fine strand detail.
%
In both industry and academia, general Monte Carlo denoising has been extensively studied using learning-based approaches, including robust average networks~\cite{kalojanov2023robust}. For hair-specific reconstruction, \citet{Currius2022} presented a CNN-based method that uses color, specular, alpha, depth, and tangent features to reconstruct hair color, specular, and alpha, but it suffers from blurring, energy variation, and high inference cost.
%
In contrast, our method employs a lightweight network to directly denoise the tangent and coverage and fill position based on them in the G-buffer, yielding better visual quality with lower runtime overhead.
